Understanding Influence Functions and Datamodels via Harmonic Analysis

Influence functions estimate effect of individual data points on predictions of the model on test data and were adapted to deep learning in Koh and Liang [2017]. They have been used for detecting data poisoning, detecting helpful and harmful examples, influence of groups of datapoints, etc. Recently, Ilyas et al. [2022] introduced a linear regression method they termed datamodels to predict the effect of training points on outputs on test data. The current paper seeks to provide a better theoretical understanding of such interesting empirical phenomena. The primary tool is harmonic analysis and the idea of noise stability. Contributions include: (a) Exact characterization of the learnt datamodel in terms of Fourier coefficients. (b) An efficient method to estimate the residual error and quality of the optimum linear datamodel without having to train the datamodel. (c) New insights into when influences of groups of datapoints may or may not add up linearly.

==> backup.tex <==
\iffalse



\begin{theorem} \label{thm:bestlinear}
    Denote the quality of a linear datamodel $(\theta,\theta_{0})\in\R^{N}\times\R$ on the $p$-biased distribution over training sets $\mathcal{B}_{p}$ by
    \begin{align}
        \mathcal{R}(\theta,\theta_{0})
        \coloneqq \mathbb{E}_{x\sim \mathcal{B}_{p}} \left[\left(f(x) - \theta_{0} - \sum_{i=1}^{N}\theta_{i} \bar{x}_{i}\right)^{2}\right].
        \label{eq:quality_linear_fit}
    \end{align}
    where $\bar{x}\in\{0,1\}^{N}$ is the binary version for any $x\in\{\pm1\}^{N}$.
    Then for $\mu = 2p-1$ and $\sigma = \sqrt{4p(1-p)}$, the following are true about the optimal datamodels with and without regularization:
    \begin{enumerate}[label=(\alph*),leftmargin=*]
        \item The unregularized minimizer $\theta^{\star},\theta^{\star}_{0} = \argmin \mathcal{R}(\theta, \theta_{0})$ satisfies
        \begin{align}
            \theta^{\star}_{i} = \frac{2}{\sigma} \wf{\{i\}}, ~~
            \theta^{\star}_{0} =  \wf{\emptyset} - \frac{(\mu+1)}{2}\sum_{i} \theta^{\star}_{i}.
            \label{eq:optimal_theta}
        \end{align}
        Furthermore the residual error is the sum of all Fourier coefficients of order 2 or higher.
       \begin{align}
            \mathcal{R}(\theta^{\star},\theta^{\star}_{0})
            = \sum_{\substack{S\subseteq[N]: |S|\ge 2}} \wf{S}^{2}
            \label{eq:residual_expression}
        \end{align}
        
        % l2 regularization
        \item The minimizer with $\ell_{2}$ regularization $\theta^{\star}(\lambda,\ell_{2}),\theta^{\star}_{0}(\lambda,\ell_{2}) = \argmin \mathcal{R}(\theta, \theta_{0}) + \lambda\|\theta\|_{2}^{2}$ satisfies
        \begin{align*}
            \theta^{\star}(\lambda,\ell_{2})_{i}
            = \frac{2}{\sigma}\left(1 + \frac{4\lambda}{\sigma^{2}}\right)^{-1} \wf{\{i\}},~~
            \theta^{\star}(\lambda,\ell_{2})_{0}
            = \wf{\emptyset} - \frac{(\mu+1)}{2}\sum_{i} \theta^{\star}(\lambda,\ell_{2})_{i}.
            \label{eq:optimal_theta_l2}
        \end{align*}
        
        % l1 regularization
        \item The minimizer with $\ell_{1}$ regularization $\theta^{\star}(\lambda,\ell_{1}),\theta^{\star}_{0}(\lambda,\ell_{1}) = \argmin \mathcal{R}(\theta, \theta_{0}) + \lambda\|\theta\|_{1}$ satisfies
        \begin{align*}
            \theta^{\star}(\lambda,\ell_{1})_{i}
            = \frac{2}{\sigma}\left(1 + \frac{4\lambda}{\sigma^{2}}\right)^{-1} \wf{\{i\}},~~
            \theta^{\star}(\lambda,\ell_{1})_{0}
            = \wf{\emptyset} - \frac{(\mu+1)}{2}\sum_{i} \theta^{\star}(\lambda,\ell_{1})_{i}.
            \label{eq:optimal_theta_l1}
        \end{align*}
    \end{enumerate}
\end{theorem}



\fi







\iffalse 
\subsection{Efficient estimate of approximation quality of datamodel} 
\label{subsec:nikunjmethod}

{\sc check against sample complexity estimate from recent paper}

Now we give a direct method (which is new, to the best of our knowledge)  to estimate  $\wf{1}^{2} =\sum_i \wf{\{i\}}^{2}$.  This gives $B_1$, and together with the easy estimate of  $\wf{\emptyset}^{2}$ immediately yields
an estimate of the residual error $B_{\geq 2}$. The method leverages that $h(\rho) = \sum_{k=1}^{N} \wf{k}^{2} \rho^{k}$ implies $h(0) = \wf{0}^{2}$ and $h'(0) = \wf{1}^{2}$.
\fi 

\iffalse 

\begin{theorem}
\label{thm:residual_estimate}
Pick independent samples $x^{(1)}, \dots x^{(n)} \in \{\pm 1\}^{N}$, from the $p$-biased distribution. The following estimate converges as $n$ increases.
\begin{align}
    B = \sum_{i=1}^{N} \wf{i}^{2}
    &= \frac{1}{n} \sum_{j=1}^{n} g(x^{(j)})^{2}\\
    B_{0} = \wf{0}^{2} / B
    &= \frac{1}{B} \frac{1}{n(n-1)} \sum_{j \neq k} g(x^{(j)}) g(x^{(k)})\\
    B_{1} = \wf{1}^{2} / B
    &= \frac{1}{B} \frac{1}{n(n-1)} \sum_{j \neq k} c(x^{(j)}, x^{(k)}) ~g(x^{(j)}) g(x^{(k)})\\
    &\text{where } ~c(x, x') = \sum_{i=1}^{N} \frac{x'_{i}(1-2p) + x'_{i}x_{i}}{1 - x'_{i} (1 - 2p)}\\
    B_{\ge2}
    &= 1 - B_{0} - B_{1}
\end{align}
\end{theorem}
%Following is a estimation procedure for $h'(0)$ given $N$ models, i.e. $N$ $x$'s sampled from the $p$-biased distribution.
\begin{proof} 
Firstly using a re-weighting trick, we note the following:
\begin{align*}
    h(\rho)
    &= \ex_{x} \ex_{x'\mid x} [g(x) g(x')]
    = \ex_{x} \ex_{x'} \left[\frac{P(x'\mid x; \rho)}{P(x')} g(x) g(x')\right]
\end{align*}
where $P(x'\mid x; \rho)$ is the $\rho$-correlated probability for $x'$ and $P(x')$ is the marginal probability. It is important to note the alternative expression $P(x') = P(x'\mid x; 0)$ since $\rho=0$ implies $x$ and $x'$ are independent. From the above expression we get
\begin{align}
    h'(\rho)
    &= \ex_{x} \ex_{x'} \left[\frac{P'(x'\mid x; \rho)}{P(x')} g(x) g(x')\right]\label{eq:h_derivate}
\end{align}
where $P'(x'\mid x; \rho) = \frac{dP(x'\mid x; \rho)}{d \rho}$.

Let $c(x, x') = P'(x'\mid x; \rho) \vert_{\rho=0}$.
Note that $P(x' \mid x; \rho) = \prod_{i=1}^{N} P(x'_{i} \mid x_{i}; \rho)$.
So
\begin{align*}
    P'(x'\mid x; \rho) \vert_{\rho=0} 
    &= \left(\sum_{i=1}^{N} P'(x'_{i} \mid x_{i}; \rho) \prod_{j\neq i} P(x'_{j} \mid x_{j}; \rho)\right)  \large\vert_{\rho=0}\\
    &= \sum_{i=1}^{N} P'(x'_{i} \mid x_{i}; \rho) \vert_{\rho=0} \prod_{j\neq i} P(x'_{j})\\
    &= P(x') \sum_{i=1}^{N} \frac{P'(x'_{i} \mid x_{i}; \rho) \vert_{\rho=0}}{P(x'_{i})}
\end{align*}
where we use chain rule for derivaters in the first step, and $P(x') = P(x'\mid x; 0)$.
Plugging this back into \Cref{eq:h_derivate} we get,
\begin{align}
    h'(0)
    &= \ex_{x} \ex_{x'} \left[c(x, x') g(x) g(x')\right]\text{, where }\\
    c(x, x')
    &\coloneqq \frac{P'(x'\mid x; \rho)\vert_{\rho=0}}{P(x')}
    = \sum_{i=1}^{N} \frac{P'(x'_{i}\mid x_{i}; \rho)}{P(x'_{i})}\label{eq:c_x_xp}
\end{align}

To compute $c(x, x')$, we first derive an expression for $P(x' \mid x; \rho)$ by looking at all the cases $x_{i}, x'_{i} \in \{+1, -1\}$, and using the $\rho$ sampling probabilities. (Using $(1+a)/2$ and $(1-a)/2$ as switches for $a=1$ and $a=-1$ respectively).
\begin{align*}
    P(x'_{i} \mid x_{i}; \rho)
    = &\frac{1+x_{i}}{2}\left[\frac{1+x'_{i}}{2}\left(1 - (1-\rho)(1-p)\right)   +  \frac{1-x'_{i}}{2}(1-\rho)(1-p)\right] + \\
    &\frac{1-x_{i}}{2}\left[\frac{1+x'_{i}}{2}(1-\rho)p   +  \frac{1-x'_{i}}{2}\left(1 - (1-\rho)p\right)\right]\\
    = &\frac{1+x_{i}}{2}\left[\frac{1}{2} + \frac{x'_{i}}{2}\left(1 - 2(1-\rho)(1-p)\right)\right] +
    \frac{1-x_{i}}{2}\left[\frac{1}{2} + \frac{x'_{i}}{2}\left(2(1-\rho)p - 1\right)\right]
\end{align*}
Note that $P(x'_{i}) = P(x'_{i}\mid x_{i}; 0) = \frac{1}{2} - \frac{x'_{i}}{2}\left(1-2p\right)$.
We now compute the derivative.
%Note that this is a linear function in $\rho$.
\begin{align*}
    P'(x'_{i} \mid x_{i}; \rho)
    &= \frac{1+x_{i}}{2} x'_{i}\left(1-p\right) - \frac{1-x_{i}}{2} x'_{i}p
    = \frac{x'_{i}}{2}(1 - 2p) + \frac{x'_{i} x_{i}}{2}
\end{align*}
Plugging this into \Cref{eq:c_x_xp}, we get
\begin{align*}
    c(x, x') = \sum_{i=1}^{N} \frac{x'_{i}(1-2p) + x'_{i}x_{i}}{1 - x'_{i} (1 - 2p)}
\end{align*}
\end{proof}
\vspace{-0.2in}

Using this estimate we find in \Cref{sec:experiments} that the residual error can be quite small for some test points, indicating a good linear fit is possible.
Notably this estimate can be with just $\sim 1000$ models with 10 seeds per model, much fewer than around 500,000 models needed by \citet{ilyas2022datamodels} to do the linear fit.
\fi 
\iffalse 
{\color{red} Estimation procedure for experiments}

Let $n$ be the training set size.
For a dataset of $n$ models, i.e. $x^{(1)}, \dots x^{(n)} \in \{\pm 1\}^{N}$, from the $p$-biased distribution, the Fourier masses can be estimated as follows:

\begin{align}
    B = \sum_{i=1}^{N} \wf{i}^{2}
    &= \frac{1}{n} \sum_{j=1}^{n} g(x^{(j)})^{2}\\
    B_{0} = \wf{0}^{2} / B
    &= \frac{1}{B} \frac{1}{n(n-1)} \sum_{j \neq k} g(x^{(j)}) g(x^{(k)})\\
    B_{1} = \wf{1}^{2} / B
    &= \frac{1}{B} \frac{1}{n(n-1)} \sum_{j \neq k} c(x^{(j)}, x^{(k)}) ~g(x^{(j)}) g(x^{(k)})\\
    &\text{where } ~c(x, x') = \sum_{i=1}^{N} \frac{x'_{i}(1-2p) + x'_{i}x_{i}}{1 - x'_{i} (1 - 2p)}\\
    B_{\ge2}
    &= 1 - B_{0} - B_{1}
\end{align}

For any $x\in\{\pm1\}^{N}$, $x_{i}$ denotes the $i^{th}$ coordinate.
\fi 

==> exact_linearity.tex <==
\subsubsection{Test for exact linearity}
\ns{Is this needed? \Cref{thm:bestlinear} and \Cref{thm:NStolinear1} already cover this. May be make it a corollary.}
\noindent{\bf Exact test for $f$ to be linear.} Now we try to understand from harmonic analysis when $f$ has a linear approximation. The following is a simple condition under which  $f$ is {\em exactly} a linear function of $x$. Note that the condition is easily tested by computing the noise stability for as few as three values of $\rho$ and checking for linearity in $\rho$.  (In practice the noise stability computation via sampling has some error and one can only conclude approximate linearity.)  
%We show this is a simple consequence of good generalization, which means that


\begin{theorem}
\label{thm:rholineariff}
Let $h(\rho)$ be as in \eqref{eqn:noise_stability}. Then $f$ is linear in $x$ iff $h$ is linear in $\rho$.
\end{theorem}
\begin{proof}
    One direction is straightforward: if $h$ is linear then $\wf{S} = 0$ whenever $|S|\ge 2$; thus only the linear terms in $f$ remain.
    For the other direction, if $f$ is linear then we want to claim that $\wf{S} = 0$ when $|S|\ge 2$ since this implies that $h$ is linear.
    We prove this by contradiction: suppose $\wf{S}>0$ for some $S$ that satisfies $|S|\ge2$.
    Let $S$ be such a set that maximizes $|S|$.
    This contributes a term $\wf{S} \sigma^{-2|S|} \prod_{i\in S} x_{i}$ to the expression of $f$.
    Note that no other basis function of the same or smaller degree can generate this monomial and cancel this term, making $f$ non-linear and leading to a contradiction.
    Thus $\wf{S}=0$ whenever $|S|\ge0$ and so $h$ is linear in $\rho$.
\end{proof}



==> fig/fig1.tex <==
\begin{figure}
\centering
    %\begin{subfigure}[b]{0.4\textwidth}
%    \includegraphics[scale=0.21]{media/figa.png}
 %   \caption{}
  %   \label{fig:1}
   % \end{subfigure}
%    \hspace*{1cm}
 %   \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[scale=0.21]{media/fig2.png}
  %  \caption{}
   % \label{fig:2}
%    \end{subfigure}
    \caption{  $h(\rho)$ versus $\rho$ for ResNet models trained on CIFAR-10. Relates to Theorem \ref{thm:rholineariff}. Each panel corresponds to a test point.  $450$ sets of $(x,x')$ were taken. Each run was averaged over 10 random seeds of SGD.$\rho=0$ and $\rho=1$ extrapolated.  }
\end{figure}

==> fig/fig2.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.5]{media/fig4.png}
    \caption{Histogram of $\bar{h}(\rho)$ for the truncated loss, $\rho = 0.5$ on 200 test points. We truncate the probability of the correct class so that if the model assigns $p \geq 1/e$ we truncate it to $p_{\text{trunc}}=1/e$. X-axis depicts $\bar{h}(\rho)$ value, and we find that for many test points their $\bar{h}(\rho)$ value is close to 1. This implies an upper bound on the quality of the linear regression as in Theorem \ref{thm:NStolinear1} }
    \label{fig:my_label}
\end{figure}


==> longtail.tex <==
\section{Harmonic analysis and  long-tail phenomenon}
\label{sec:longtail}
We recall interesting empirical discoveries from~\cite{feldman2020does} and \cite{feldman2020neural}. %gave empirical evidence for the {\em long tail phenomenon}. 
{\em Memorization phenomenon} says that for a significant fraction of training points, the model does not learn to predict their labels very well if they are omitted from training set. As noted in~\cite{feldman2020does}  this can be seen as a sort of "self-influence". For the $i$th training datapoint, let $f(x)$ be the probability that the model trained on $f$ predicts the correct label for $i$ when trained using dataset $x$. Memorization is said to happen for $i$ if for a reasonably large $p$ like $0.5$ or $0.7$, the following holds with reasonable probability over $p$-biased $x$ in which $x_i =-1$:
\begin{equation} f(x|_{i \rightarrow 1}) - f(x) > 0.3. \end{equation}
(Here $0.3$ is used just for example.) In other words, the model trained on $p$ fraction of datapoints  does not learn to classify $i$ very well if $i$ is not part of the training set. 
%It was discovered that a significant fraction of the training set has this property, which suggests a 
The related {\em long tail} phenomenon is that prediction on a few percent of test points is fragile in the sense that each can be misclassified if a small number of memorized training points are omitted.% (with are found to be "memorized" on ``typical'' training data points. 

%Furthermore,  the authors then present evidence that a few percent of  test points  are difficult to classify, in the sense  that ability to classify them well depends on presence of a small number of such non-typical training points during training. 

\looseness-1 Note that this entire understanding is based upon experiments. While it feels intuitive (especially due to use of  terms like ``influence'')  that classifying the long tail ``depends'' on the presence of a few influential points, it is not immediately clear how to capture this phenomenon at a mathematical level. Concretely, suppose $f_1(x)$ is the probability of correctly classifying a fixed test point $z_1$ on a $p$-biased training set  $x$. Suppose we have computed the influences of individual training datapoints for $f_1$, and found only a small number of these to be significant, thus marking it as ``long tail." As compared to test function $f_2(x)$ associated for a typical test point $z_2$, where we don't find any single training point which has a large influence on $f_2$. In what sense is %are the two test points $z_1$ and $z_2$ different based upon this information? In what sense is 
$z_1$ ``harder'' to classify than $z_2$ based upon this information? 

As usual, complete answer awaits full mathematical understanding of every component of deep learning, but  a rough answer emerges from harmonic analysis when we focusing on the derivative with respect to $p$:  how quickly does $f$ improve as we increase the bias parameter $p$ that defined $x$? In other words, how quickly does $f$ improve with growth in the training set? This study is most interesting around a $p$ where the probability (over choice of $x$ from the $p$-biased distribution) of the correct label is bounded away from both $0$ and $1$. We capture this by assuming the variance of $f(x)$ is a constant. (Our experiments in Section~\ref{sec:experiments} show examples of how $f$ changes with $p$ in this region for different test points. 

The following definition is crucial. Our experiments with the methods for estimating
the quality of the linear datamodel (Section~\ref{subsec:nikunjmethod}) suggest that it holds for reasonable constant $C_2$ in the region of interest. 

\begin{definition}[$C_2$-linear function]
Let $f$ be a function and $\tilde{f}(p)$ be the average value of $f_j$  and $Var_{f}(p)$ be the variance of $f$ over $x\sim B_p^n$. We say it is $C_2$-linear if at least $C_2$ fraction of the variance is explained by the linear term, that is:
$$
\sum_{i} \widehat{f_{{\{i\}}}}^2\ge C_2 \cdot Var_{f}(p).
$$
\end{definition}
\vspace{-0.2in}

Next definition  is motivated by the following, which
uses \cref{eqn:influencei}:
\begin{align}
    \overline{\text{Inf}}_i^1(f)& = \mathbbm{E}_{x_{-i}\sim B_p} \left[ 
    f(x_{-i},x_i=1)-f(x_{-i},x_i=-1)\right]  
     = c_p \widehat{f_{\{i\},p}}
\end{align}
\begin{definition}[Monotone on average] We say $f$ is monotone on average if $\overline{\text{Inf}}_i^1(f)$ is nonnegative for
all $i$.
\end{definition}
In practice, monotonicity probably does not completely hold for all $i$, but for most. (Failure of monotonicity would be expected for  training points that are mislabeled or have ambiguous labels.) 

% Adjusting for this is left for future work.  
%\begin{theorem} 
%Let $f_1, f_2$ be functions as above that are $C_2$-linear for some constant $C_2>0$.
%$\tilde{f_j}(p)$ be the average value of $f_j$  and $Var_{f_j}(p)$ be the variance of $f_j$ over $x\sim B_p^n$. Suppose that at least $C_2$ fraction of the variance is explained by the linear term, that is:
%$$
%\sum_{i} \widehat{f_{j,{\{i\},p}}}^2\ge C_2 \cdot Var_{f_j}(p).
%$$Suppose that at least $C_2$ fraction of the variance is explained by the linear term, %that is:
%$$
%\sum_{i} \widehat{f_{j,{\{i\},p}}}^2\ge C_2 \cdot Var_{f_j}(p).
%$$
The next theorem shows (assuming $\varepsilon$ is negligible, or at least the total influence of the ``irrelevant'' $i$'s is negligible) that for the same (classification performance, variance) profile, ``long-tail" functions such as $f_1$ grow much more slowly as we increase $p$. By contrast, functions like $f_2$ quickly shoot up as $p$ is increased. Experiments in Section~\ref{sec:experiments} shows some examples of both types, confirming this prediction. 
\begin{theorem}
\label{thm:longtail}
Let  $f_1(x), f_2(x)$ be as defined above. Assume $f_2$ is monotone on average. Let $c_p = 2\sqrt{\frac{1-p}{p}}$.
\begin{enumerate}
    \item 
    Suppose $f_1$ has at most $C_1$ training points with influence $> \varepsilon$. (These are points such that adding them to the training set improves success probability by more than $\varepsilon$ in expectation.) Then 
    \begin{equation}
     \frac{d\tilde{f_1}(p)}{dp} < C_1 +\varepsilon\cdot N
    \end{equation}
\item 
Suppose $f_2$ is $C_2$-linear for some constant $C_2$ and every training datapoint $i$ has influence at most $\delta_2$. Then,
    \begin{equation}
     \frac{d\tilde{f_2}(p)}{dp} \ge  \frac{C_2 \cdot Var_{f_2}(p)}{\delta_2 \cdot c_p},
    \end{equation}
    in other words, the derivative is inversely proportional to $\delta_2$
\end{enumerate}
\end{theorem}

\begin{proof}
\looseness-1 We begin with some general calculations, which we then use to obtain the two bounds. Note that 
\begin{equation}
    \tilde{f}(p):=\mathbbm{E}_{x_i\sim B_p}[f(x)] = \widehat{f_{\emptyset,p}}. 
\end{equation}
%In addition, whenever $f$ is monotone, we have 

We also have
\begin{equation}
    \frac{d\tilde{f}(p)}{dp} = 
    \sum_{i=1}^n  \overline{\text{Inf}}_i^1(f) = c_p \sum_{i=1}^n  \widehat{f_{\{i\},p}} \label{eq:ell1}
\end{equation}

Hence we obtain
\begin{align*}
 \frac{d\tilde{f}(p)}{dp} & = 
    \sum_{i=1}^n  \overline{\text{Inf}}_i^1(f) \qquad = \sum_{i \in \text{influential}}
    \overline{\text{Inf}}_i^1(f)  +\sum_{i\notin\text{influential} }
    \overline{\text{Inf}}_i^1(f) \\ & \le |\text{influential}| + \varepsilon\cdot n \qquad  \le C_1 + \varepsilon\cdot N.
\end{align*}

Next, we turn our attention to the second statement. By assumption,
$
\sum_{i} \widehat{f_{j,{\{i\},p}}}^2\ge C_2 \cdot Var_{f_j}(p).
$
Also   
$\delta_2 \ge c_p\widehat{f_{\{i\},p}}$
and therefore $\widehat{f_{\{i\},p}}\le \delta_2 \cdot c_p^{-1}$. Together with $\widehat{f_{\{i\},p}}\ge 0$, and the fact that $Inf_i^1(f)\le 1$ for all $i$ (since $f_1, f_2$ take values in $[0,1]$) we get
\begin{align*}
     \frac{d\tilde{f}(p)}{dp} & =  \sum_{i=1}^n c_p \widehat{f_{\{i\},p}} \qquad \ge c_p \sum_{i=1}^n \widehat{f_{\{i\},p}}^2
     \qquad   \ge \frac{C_2 \cdot Var_{f_j}(p)}{c_p\delta_2}
\end{align*} \end{proof}
\vspace{-0.2in}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> table/algo0.tex <==
\begin{algorithm}
\caption{Efficient algorithm for residual estimation \ns{better formatting needed}}\label{alg:residual_est}
\KwData{Function $f$, function eval budget $n$, list $[\rho_{1}, \dots, \rho_{k}]$, degree $d$, $solver$ (`linear' or `convex')}
$\bm{y} \in \mathbb{R}^{k}$

$\bm{A} \in \R^{k \times (d+1)}$

\For{$i \in [1, \dots, k]$} {
    $\bm{y}[i] \gets \text{NoiseStability}(f, n/k, \rho_{i})$\\
    $\bm{A}[i,:] \gets [1, \rho_{i}, \dots, \rho_{i}^{d}]$
}
\eIf{$solver == \text{`linear'}$ and $k \ge d+1$}{
    Solve $\hat{\bm{z}} = \min_{\bm{z}\in\R^{d+1}} \|\bm{A}\bm{z} - \bm{y}\|_{2}^{2}$
}
{
    Solve $\hat{\bm{z}} = \min_{\bm{z}\in\R^{d+1}} \|\bm{A}\bm{z} - \bm{y}\|_{2}^{2} \text{ s.t. } \bm{z}\ge\bm{0}$
}

$\hat{B}_{0} \gets \bm{z}[1]$

$\hat{B}_{1} \gets \bm{z}[2]$

$\hat{B} \gets \text{NoiseStability}(f, n/k, 1)$

Return $\hat{B} - \hat{B}_{0} - \hat{B}_{1}$
% $x \in \R^{d}$ /* Corresponding to $x_{i} = \hat{B}_{i}$ */
\end{algorithm}

==> table/table1.tex <==
\begin{table}
\caption{Values of $B0$, $B_1$, and $B_2$ for CIFAR-10 data provided by \cite{ilyas2022datamodels}. Estimated using procedure in Section \ref{subsec:nikunjmethod}, Training masks are of size 5000. Each row represents a test point. We find that the residuals are not too large. }
\label{table:ilyas}
\begin{tabular}{||c c c c||} 

 \hline
 Test point index & $B_0$ & $B_1$ & $B_{\geq 2}$\\ [0.5ex] 
 \hline\hline
 3001 & 0.70 & 0.36 & -0.06 \\ 
 \hline
 3002 & 0.45 & -0.15 & 0.70 \\
 \hline
 3003 & 0.56 & 0.13 & 0.31 \\
 \hline
 3004 & 0.42 & 0.41 & 0.17 \\
 \hline
 3005 & 0.44 & 0.44 & 0.11 \\ [1ex] 
 \hline
\end{tabular}

\end{table}

==> table/table2.tex <==
\begin{table}

\caption{Values of $B0$, $B_1$, and $B_2$ for CIFAR-10 data with our trained models for selected test points. Estimated using procedure in Section \ref{subsec:nikunjmethod}. Average value of probability of correct class taken over 10 random seeds. $p=0.1$. Each row is a test point. }
\label{table:our}
\begin{tabular}{||c c c c||} 

 \hline
 & $B_0$ & $B_1$ & $B_{\geq 2}$\\ [0.5ex] 
 \hline\hline
 & 0.916 & 0.065 & 0.0185 \\ 
 \hline
 & 0.931 &  0.065 &  0.0025 \\
 \hline
  & 0.905 & 0.0518 & 0.0429 \\
 \hline
  & 0.959 & 0.000861 & 0.0400 \\
 \hline
  &  0.895 & 0.108 & -0.0413 \\ [1ex] 
 \hline
\end{tabular}

\end{table}
